AdaPool: A Diurnal-Adaptive Fleet Management Framework using Model-Free Deep Reinforcement Learning and Change Point Detection

This paper introduces an adaptive model-free deep reinforcement approach that can recognize and adapt to the diurnal patterns in the ride-sharing environment with car-pooling. Deep Reinforcement Learning (RL) suffers from catastrophic forgetting due to being agnostic to the timescale of changes in the distribution of experiences. Although RL algorithms are guaranteed to converge to optimal policies in Markov decision processes (MDPs), this only holds in the presence of static environments. However, this assumption is very restrictive. In many real-world problems like ride-sharing, traffic control, etc., we are dealing with highly dynamic environments, where RL methods yield only sub-optimal decisions. To mitigate this problem in highly dynamic environments, we (1) adopt an online Dirichlet change point detection (ODCP) algorithm to detect the changes in the distribution of experiences, (2) develop a Deep Q Network (DQN) agent that is capable of recognizing diurnal patterns and making informed dispatching decisions according to the changes in the underlying environment. Rather than fixing patterns by time of week, the proposed approach automatically detects that the MDP has changed, and uses the results of the new model. In addition to the adaptation logic in dispatching, this paper also proposes a dynamic, demand-aware vehicle-passenger matching and route planning framework that dynamically generates optimal routes for each vehicle based on online demand, vehicle capacities, and locations. Evaluation on New York City Taxi public dataset shows the effectiveness of our approach in improving the fleet utilization, where less than 50% of the fleet are utilized to serve the demand of up to 90% of the requests, while maximizing profits and minimizing idle times.

==> AdaPool.tex <==
\section{Methodology} \label{work}
We consider the scenario where the environment changes between models $1, 2, ...., n$ dynamically. The implication of the non-stationary environment is this: when the agent exercises a control $a_{t}$ at time $t$, the next state $s_{t+1}$ as well as the reward $r_{t}$ are functions of the \textit{active} environment model dynamics. In our approach, we assume the knowledge of the pattern of change in the environemnt models $M_{1}, M_{2}, .... M_{n}$. However, neither  the context information of each model nor the change points $T_{1}, T_{2}, ...$, etc., when these model changes occur, are known to the RL agent. In this case, the agent can collect experience tuples while simultaneously following a model-free learning algorithm to learn an approximately optimal policy. Instead of assuming any specific structure, our model-free approach learns the Q-values dynamically using convolutional neural networks. Our method works in tandem with a change point detection algorithm, to get information about the changes in the environemnt. Then, it updates Q-values of the relevant model whenever a change is detected and does not attempt to estimate the transition and reward functions for the new model. Additionally, if the method finds that samples are obtained from a previously observed model, it updates the Q values corresponding to that model. Thus, in this manner, the information which was learnt and stored earlier (in the form of Q-values) is not lost.

%We utillize this framework in \cite{deep_pool} to re-balance vehicles over the city to better serve the demand. At the beginning of every time step $t$, vehicles that newly enter the system at time $t$, are dispatched to areas of anticipated high demand follwoing this approach. Moreover, at the end of every time step, we check for vehicles whose idle duration exceeds 10 minutes, and we apply this technique to dispatch them to high-demand areas to better utilize our resources.

The learning begins by obtaining experience tuples $E_{t}$ according to the dynamics and reward function of current active model $M_{\theta_{c}}$ . The state and reward obtained are stored as experience tuples, since model information is not known. The samples can be analyzed for context changes in batch mode or online mode. If a change gets detected, then the counter $c$ is incremented, signalling that the
agent believes that context has changed. We adapt the online parametric Dirichlet changepoint (ODCP) detection algorithm proposed in \cite{7-ada} for data consisting of experience tuples. This algorithm transforms any discrete or continuous data into compositional data and utilizes Dirichlet parameter likelihood testing to detect change points. Multiple changepoints are detected by performing a sequence of single changepoint detections. Although ODCP requires the multivariate data to be i.i.d samples from a distribution. The justification in \cite{9-ada} explains the utilization of ODCP in the Markovian setting, where the data obtained does not consist of independent samples.

At every time step $t$, the DQN agent obtains a representation for the environment, $s_{t, n}$, and calculates a reward $r_{t}$ associated with each dispatch-to location in the action space $a_{t, n}$ according to the dynamics and reward function of current active model $M_{\theta_{c}}$. Based on this information, the agent takes an action that directs the vehicle to different dispatch zone where the expected discounted future reward is maximized. In our algorithm, we define the reward $r_{k}$ as a weighted sum of different performance components that reflect the objectives of our DQN agent. The reward will be learnt from the environment for individual vehicles and then leveraged by the agnet/optimizer to optimize its decisions. 

We define the overall objectives of the dispatcher, where our dispatch policy aims to (1) minimize the supply-demand mismatch: ($\text{diff}_{t}$), (2) minimize the dispatch time: $T_{t}^{D}$ (i.e., the expected travel time of vehicle $V_{j}$ to go zone $m$ at time step $t$), (3) minimize the extra travel time a vehicle takes for car-pooling compared to serving one customer: $\Delta t$, (4) maximize the fleet profits $P_{t}$, and (5) minimize the number of utilized vehicles: $e_{t}$. We capture this by minimizing the number of vehicles that become active from being inactive at time step $t$. %Although we are minimizing the number of active vehicles in time step $t$, if the total distance or the total trip time of the passengers increase, it would be beneficial to use an unoccupied vehicle instead of having existing passengers encounter a large undesired delay. 
The DQN overall reward function is represented as a weighted sum of these terms for individual agents/vehicles:
\begin{equation} \label{individual}
\begin{multlined}
r_{t, n} = r(s_{t,n}, a_{t,n})
= \beta_{1} C_{t,n} + \beta_{2} T_{t,n}^{D} + \beta_{3} T_{t,n}^{E} + \beta_{4} \mathbb{P}_{t,n} + \\ \beta_{5} [\text{max}(e_{t,n} - e_{t-1,n}, 0)]
\end{multlined}
\end{equation}

%Through learning the probabilistic dependence between the action and the reward function, we learn the Q-values according to the dynamics and reward function of current active model $M_{\theta_{1}}$ associated with the probabilities $P(r_{t}\mid a_{t},s_{t})$ over time by feeding the current states of the system. The Q-values are then used to decide on the best dispatching action to take for each individual vehicle.

%Note that the additional profits term $P_{t}$ integared with the reward function makes the output expected discounted rewards (Q-values) associated with each possible move on the map, a good reflection of the expected earnings gained when heading to these locations. This gives drivers an insight about how the supply-demand is distributed over the city, and assists them in making knowledgeable and informed dispatching decisions.


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> dprs.tex <==
In this section, we elaborate the pricing-based strategy components that are built on top of the distributed ride-sharing environment detailed in Section \ref{joint}. In our simulator setup, we consider various vehicle types: hatch-back, sedan, luxury, and van. Each of which has different capacity, mileage, and base price for driver per trip denoted by $B_{j}$. $B_{j}$ serves as the local minimum earning that the driver gains per trip. Also, based on the vehicle type, the pricing per mile distance varies as well as the pricing per waiting minute.

\subsection{Initial Pricing} \label{init_price}
Initially, the system suggests a price for each vehicle-customer matching, taking into consideration several factors:
\begin{itemize}[leftmargin=*]
	\item The total trip distance, i.e., the distance till pickup plus the distance from pickup to drop off. Note that, this distance is composed of the weights of the $n$ edges that constitute the vehicle's optimal route from its current location to origin $o_{i}$ and then to destination $d_{i}$. This is obtained as explained in Algorithm \ref{insert}, as the cost associated with route $S_{V_{j}} = [loc(V_{i}), o_{i}, d_{i}]$ after inserting request $r_{i}$ into vehicle $V_{j}$'s current route, assuming initially that $r_{i}$ is the only request matched to vehicle $V_{j}$. Thus, cost($V_{j}, S_{V_{j}[r_{i}]}$) after subtracting the cost of the original route before insertion. Then, in the next step when driver already knows the updated route $S^{\prime}_{V_{j}}$ , they plug into the equation cost($V_{j}, S^{\prime}_{V_{j}[r_{i}]}$).
	\item Number of customers who share travelling a trip distance (whether all or part of it, which can be determined from the vehicle's path). For simplicity, we denote it by the vehicle $j$'s capacity $V^{j}_{C}[o_{i}]$ when it reaches the origin $o_{i}$ location of this request $r_{i}$ subtracted from its capacity when it reaches the destination $d_{i}$, $V^{j}_{C}[d_{i}]$. Thus, we define $V^{j}_{C}[r_{i}] = \; \mid V^{j}_{C}[d_{i}] - V^{j}_{C}[o_{i}] \mid$. Initially, this is just an estimation, using the number of requests in the initial matching $A_{j}$ assigned to vehicle $V_{j}$ at timestep $t$. However, at the destination where the customer is expected to make the payment, all these numbers become already known (i.e. deterministic exact values).
	\item The cost for fuel consumption associated with this trip, denoted by $D_{i}*(P_{gas}/M_{j})$, where $P_{gas}$ represents the average gas price, and $M^{j}_{V}$ denotes the mileage for vehicle $j$ assigned to trip $i$.
	\item The waiting time experienced by the customer (or customers) associated with trip $i$ till pickup, denoted $T_{i}$.
\end{itemize}
The overall price initialization equation for request $r_{i}$ is represented as:
\begin{equation}\label{init}
\begin{multlined}
P_{init}[r_{i}] = B_{j} + \left[ \omega^{1}*\frac{cost(V_{j}, S_{V_{j}[r_{i}]})}{V^{j}_{C}[r_{i}]} \right] \; \\ +\; \left[ \omega^{2}* \left( \frac{cost(V_{j}, S_{V_{j}[r_{i}]})}{V^{j}_{C}[r_{i}]}*(P_{gas}/M^{j}_{V}) \right) \right] \; - \; \left[ \omega^{3}*T_{i} \right]
\end{multlined}
\end{equation}
where $\omega^{1}, \omega^{2}$, and $\omega^{3}$ are the weights associated with each of the factors affecting the price calculation. $\omega^{1}$ is the price per mile distance according to the vehicle type. $\omega^{2}$ is set to 1 as it doesn't change across vehicles, what changes is the mileage in this factor. Finally, $\omega^{3}$ is the price per waiting minute that is influenced by the vehicle type, it is negative here as we want to minimize the waiting time for the customer. %Note that, our framework runs in two modes. A customer can select either to carpool or not. If the customer decides not to carpool, the vehicle will not pickup any extra customers until this customer drops off, and thus $V^{j}_{C}$ will always be 1. However, for ride-sharing customers: the path for trip $i$, $D_{i}$ is composed of $k$ routes: $D_{i} = \sum^{k}_{i=1} r_{i}$. So, for each customer, $D_{i}$ will be the sum of distances of the shared routes among other customers, with $V^{j}_{C}$ set to the number of customers to ride-share with. Then, the price for the remaining non-shared distance, if any, will be calculated with $D_{i}$ equals to the sum of distances of all un-shared routes and $V^{j}_{C} = 1$. The sum of both will constitute the total initial pricing. This initial pricing gets updated for on-board passengers whenever a vehicle picks up an additional customer (as the $V^{j}_{C}$ will now increase), where all the overlapping (shared) distances are taken into consideration (when constructing $D_{i}$) and thus price may get reduced. 
Our proposed algorithm will first use the initial price and notify the vehicle (or driver), who will then modify the pricing based on the Q-values of the driver's dispatch-to location.

\subsection{Vehicles' Proposed Pricing} \label{propose}
Each driver follows a dispatch policy once he/she enters the market. This dispatch policy provides him/her with the best next dispatch action to make, which is predicted after weighing the expected discounted rewards (Q-values) associated with each possible move on the map using DQN (described in Section \ref{dqn_algo} and Appendix \ref{dqn}). As a result of running such a policy every dispatch cycle (which is set to 5 minutes), the driver gains insight about how the supply-demand is distributed over the city, and thus can make informed decisions on which destinations can yield him a higher profit. The vehicle's (or driver's) decision-making process is formulated as follows:

\begin{itemize}[leftmargin=*]
	\item Based on the knowledge of the expected discounted reward (i.e. Q-values) associated with the action of going to each location on the map (i.e. using DQN to learn the Q-values associated with each action), the driver can order the destinations in a descending order and assign each of them a rank $\alpha$, representing where it falls in that ordered list. The driver dynamically maintains this ranking and continuously updates it whenever the dispatch policy runs. For flexibility, the driver also has a tolerance rate, $\lambda$ (which is a percentage), that he/she uses to decide on the size of the \textit{desired zones} list.
	\item After the route planning optimization step, the driver re-calulates the initial pricing $P_{init}(r_{i})$ using the updated route $S^{\prime}_{V_{j}}$ , by plugging cost($V_{j}, S^{\prime}_{V_{j}[r_{i}]}$) (after subtracting the cost of the original route before insertion) into equation \ref{init}. This is done to account for any detours required to serve this new request $r_{i}$, and thus enforces requests going in the same direction to be matched together.

	\item Knowing the request pickup location, the driver retrieves the ranking $\alpha$ associated with various destinations. After that, he adds the highest ranking $\lambda$ locations to a set of \textit{desired zones}, denoted $L$. Then, if the request's location is among that desired set $L$, the driver uses the initial pricing suggested for this trip, denoted $P_{init}(r_{i})$.
	\item Otherwise, it would indicate that he/she might end up in the middle of nowhere (region with low demand), and thus receives no more requests or at least drives idle a long distance. Instead of just rejecting the request, he/she can suggest a price to the customer that is slightly higher by a factor influenced by both the rank of the destination as well as his/her own base price per trip $B_{j}$.  
\end{itemize} 

Let $P(r_{i})$ represents the final price suggested by driver $j$ for the customer associated with request/trip $i$, the driver's price decision is as follows:
\begin{equation} \label{car}
P(r_{i}) = \begin{cases}
P_{init}(r_{i}) &\text{if $loc(r_{i}) \in L$}\\
P_{init}(r_{i}) +  \\ [P_{init}(r_{i}) *\frac{\alpha_{loc(r_{i})}}{2}*B_{j}] &\text{otherwise}
\end{cases}
\end{equation}

\subsection{Customers' Decision Function}\label{decide}
After the driver makes a decision regarding the price associated with the trip, it becomes the customer's turn to make his/her own decision according to his/her set of preferences. In our algorithm, we consider various preferences for each customer:
\begin{itemize}[leftmargin=*]
	\item Whether the customer is in a hurry or not or how much delay can he/she tolerate. This is taken into consideration in the customer's utility  and denoted by delay/waiting time of trip $i$: $T_{i}$.
	\item Whether the customer prefers car-pooling or would rather take the ride alone even if it means a higher price. This is captured in the utility equation based on the current capacity of vehicle $j$ assigned to trip $i$, denoted by $V^{j}_{C}$.
	\item Whether he/she prefer a certain type of vehicle for their trip, and whether he/she is willing to par more in exchange for a more luxurious vehicle. The type of vehicle $j$ assigned to trip $i$ is denoted by $V^{j}_{T}$.
\end{itemize} 
Based on the aforementioned factors, the customer's utility for request/trip $i$ is formulated as:
\begin{equation} \label{customer1}
U_{i} = \left[ \omega^{4} * \frac{1}{V^{j}_{C}} \right] + \left[ \omega^{5} * \frac{1}{T_{i}} \right] + \left[ \omega^{6} * V^{j}_{T} \right]
\end{equation}

where $\omega^{4}, \omega^{5}$, and $\omega^{6}$ are the weights associated with each of the factors affecting the customer's overall utility. To add more flexibility, we introduce a customer's compromise threshold $\delta_{i}$ to represent how much the customer $i$ is willing to compromise in the decision-making process. Finally, the decision of customer $i$ to accept or reject, denoted by $C^{i}_{d}$, after receiving the final price $P(r_{i})$ for the trip $i$ is as follows:
\begin{equation}\label{customer2}
C^{i}_{d} = \begin{cases}
1 &\text{if $ U_{i} > P(r_{i}) - \delta_{i}$}\\
0 &\text{otherwise}
\end{cases}
\end{equation}

Upon customer's acceptance, no further action is required, and the process continues. In case of rejection, a new matching process is initiated to match this request to another vehicle that better meets their preferences.
